Sequential Deep Learning Architectures for Anomaly Detection in Virtual Network Function Chains

Software-defined networking (SDN) and network function virtualization (NFV) have enabled the efficient provision of network service. However, they also raised new tasks to monitor and ensure the status of virtualized service, and anomaly detection is one of such tasks. There have been many data-driven approaches to implement anomaly detection system (ADS) for virtual network functions in service function chains (SFCs). In this paper, we aim to develop more advanced deep learning models for ADS. Previous approaches used learning algorithms such as random forest (RF), gradient boosting machine (GBM), or deep neural networks (DNNs). However, these models have not utilized sequential dependencies in the data. Furthermore, they are limited as they can only apply to the SFC setting from which they were trained. Therefore, we propose several sequential deep learning models to learn time-series patterns and sequential patterns of the virtual network functions (VNFs) in the chain with variable lengths. As a result, the suggested models improve detection performance and apply to SFCs with varying numbers of VNFs.

==> bkup.tex <==

% explanation about each model
For the first set of experiments, we aim to measure the anomaly detection performances of our models using different encoder networks. Each models were trained on train set, then tested its performance in web service scenario dataset as in table \ref{tbl:basic_result} and in login authentication scenario as in table \ref{tbl:basic_result2}. In order to show the effectiveness of using encoder model, we experimented with model which uses no encoder. For this model, we preprocess raw input data and directly apply readout layer. For all other models, preprocessed input data go through encoder network to obtain contextualized output vectors.

% basic experiment result and graph
\begin{table}[h!] \centering	
\caption{Experiment result of encoder + classifier models on web service scenario using 200ms resp. time, 99.95\% availability SLA criteria. For each model, the input data sequence was encoded by encoder network and then fed into classifier network. 'no-enc' model takes raw input sequence directly to readout layer and input into classifier network.}
    \label{tbl:basic_result}
    \begin{tabular}{| l | r |}
    \hline
    \textbf{ Model } & \textbf{ f1-measure } \\ \hline \hline
   no-enc & 0.9264 \\
   RNN-enc & 0.9524 \\
   Bi-RNN-enc  & 0.9496 \\
   Transformer-enc  & 0.9534 \\
   GNN-enc & 0.9442 [20.12.24.exp1] \\
   \hline
   \end{tabular}
\end{table}

\begin{table}[h]
\centering
    \caption{Experiment result of encoder + classifier models on login authentication scenario using 200ms resp. time, 99.95\% availability SLA criteria. 'no-enc' model takes raw input sequence directly to readout layer and input into classifier network.}
    \label{tbl:basic_result2}
        \begin{tabular}{lll}
            \textbf{ Datasets } & \textbf{ Models } & \textbf{ f1-measure } \\ \hline \hline
            \multirow{4}{*}{250ms resp. time, 99.95\% availability} & \multicolumn{1}{l}{no-enc} & \multicolumn{1}{l}{0.8603} \\\cline{2-3}
                                 & \multicolumn{1}{l}{RNN-enc} & \multicolumn{1}{l}{0.9331} \\\cline{2-3}
                                 & \multicolumn{1}{l}{Bi-RNN-enc} & \multicolumn{1}{l}{0.9364} \\\cline{2-3}
                                 & \multicolumn{1}{l}{Transformer-enc} & \multicolumn{1}{l}{0.9416} \\\cline{2-3}
                                 & \multicolumn{1}{l}{GNN-enc} & \multicolumn{1}{l}{0.9268} \\\hline
            \multirow{4}{*}{200ms resp. time, 99.99\% availability} & \multicolumn{1}{l}{no-enc} & \multicolumn{1}{l}{0.8236[20.12.24.exp3]} \\\cline{2-3}
                                 & \multicolumn{1}{l}{RNN-enc} & \multicolumn{1}{l}{0.8894} \\\cline{2-3}
                                 & \multicolumn{1}{l}{Bi-RNN-enc} & \multicolumn{1}{l}{0.8996} \\\cline{2-3}
                                 & \multicolumn{1}{l}{Transformer-enc} & \multicolumn{1}{l}{0.9004} \\\cline{2-3}
                                 & \multicolumn{1}{l}{GNN-enc} & \multicolumn{1}{l}{0.8755[20.12.24.exp3]} \\\hline
        \end{tabular}
\end{table}

% RNN direction
% default hyper-parameter for RNN model
% relation to Bi-RNN model
% The direction of 

% some observations from the result
For results, using encoder network showed better result than not using encoder network as shown in tables \ref{tbl:basic_result} and \ref{tbl:basic_result2}.
Bi-RNNs and Transformer networks generally shows better performance in NLP field as they have capacity to encode more various and complex temporal patterns. Our experiment result is in line with this general results where performance of Bi-RNNs surpasses that of RNNS while Transformer shows even better performance.

% what could be experimented more?
Since one of contributions of our proposed model is scalability, we experimented more detailed performance about scalability of our models. We also propose joint training method to increase scalability of our proposed models. Furthermore, since our models have various hyper-parameters which could have large effects on performance, we  selected a set of hyper-parameters such as number of layers and show correlation of model performance with respect to values of them. Lastly, we carries out automatic hyper-parameter tuning framework to search the best hyper-parameter settings. Then we compare the performance with models which did not use encoder network and analyze the benefits of our model.


%%% table for concatenation-based models
\begin{figure}[h]
\centerline{\hbox{ 
\includegraphics[width=3.4in]{experiment_result1.png}
%\hspace{0.05in}
}}
\caption{Experiment result 1}
\label{fig:experiment_result1}
\end{figure}

\begin{table}[h!] \centering	
\caption{ Baseline models that use concatenated features to detect anomaly. these models are not scalable to varying number of nodes. }
    \label{tbl:non-scalable_baseline}
    \begin{tabular}{| l | r | r | r |}
    \hline
    \textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{f1-measure}  \\ \hline \hline
    DNN & 0.xxxx & 0.xxxx & 0.xxxx\\ 
    Random Forest & 0.xxxx & 0.xxxx & 0.xxxx\\
    Naive Bayes & 0.xxxx & 0.xxxx & 0.xxxx\\
    KNN  & 0.xxxx & 0.xxxx & 0.xxxx\\
    SVM & 0.xxxx & 0.xxxx & 0.xxxx\\
   \hline
   \end{tabular}
\end{table}


\begin{figure*}[h]
\centerline{\hbox{ 
\includegraphics[width=6.8in]{scalability_result.png}
%\hspace{0.05in}
}}
\caption{Scalability results. (a) performance over web service scenario environment. (b) performance over login authentication scenario environment. The experiment was carried out over datasets with 200ms resp. time, 99.95\% availability SLA criteria. We plan to carry out more experiments over different SLA criteria in the future works.}
\label{fig:scalability_result}
\end{figure*}

\begin{table}[h!] \centering	
\caption{Scalability of encoder + classifier models on login authentication scenario using 200ms resp. time, 99.95\% availability SLA criteria.}
    \label{tbl:scalability_2}
    \begin{tabular}{| l | r | r | r | r |}
    \hline
    \textbf{ Model } & \textbf{ default } & \textbf{ method 1 } & \textbf{ method 2 } \\\hline \hline
   no-enc & 0.8456 & 0.6363 & 0.8277 \\
   RNN-enc & 0.9055 & 0.7425 & 0.8911 \\
   Bi-RNN-enc  & 0.9010 & 0.7450 & 0.8775 \\
   Transformer-enc  & 0.8956 & 0.7124 & 0.8940 \\
   GNN-enc [20.12.24.exp3] & 0.8755 & 0.7015 & 0.xxxx \\
   \hline
   \end{tabular}
\end{table}

\begin{table*}[!h]
  \centering
    \caption{Scalability evaluation results for different models}
    \label{tbl:scalability_2}
  \begin{tabular}{|c|c|c|ccc|ccc|c|}
    \hline
      \multirow{3}{*}{\bfseries Training dataset} & \multirow{3}{*}{\bfseries Encoder} & \multirow{3}{*}{\bfseries Readout} & \multicolumn{6}{|c|}{\bfseries Test dataset} & \multirow{3}{*}{\shortstack[*]{\bfseries Average\\\bfseries F1-measure}} \\
      \cline{4-9}
      & & & \multicolumn{3}{|c|}{\bfseries WSD} & \multicolumn{3}{|c|}{\bfseries LAD2} & \\
    \cline{4-9}
    % \bfseries Testset  & \bfseries Encoder & \bfseries Readout 
    & & & \bfseries Precision & \bfseries Recall & \bfseries F1-measure & \bfseries Precision & \bfseries Recall & \bfseries F1-measure & \\
    \hline\hline
    
    \multirow{4}{*}{\bfseries WSD} & GG-NN & \multirow{4}{*}{\shortstack[c]{Max / Mean /\\Self-attention }} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\\cline{2-2}\cline{4-10}
    & RNN & & 95.45 & 94.60 & 95.02 & 78.37 & 70.59 & 74.25 & 84.64\\\cline{2-2}\cline{4-10}
    & Bi-RNN & & 95.41 & 95.10 & 95.25 & 78.85 & 70.63 & \underline{74.50} & \underline{84.88} \\\cline{2-2}\cline{4-10}
    & Transformer & & 95.34 & 95.42 & \textbf{95.38} & 71.41 & 71.40 & 71.24 & 83.31  \\\hline\hline
    
    \multirow{4}{*}{\bfseries LAD2} & GG-NN & \multirow{4}{*}{\shortstack[c]{Max / Mean /\\Self-attention}} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\\cline{2-2}\cline{4-10}
    & RNN & & 68.33 & 80.23 & 73.79 & 93.36 & 87.94 & \underline{\textbf{90.55}} & 82.17  \\\cline{2-2}\cline{4-10}
    & Bi-RNN & & 65.79 & 82.27 & 73.09 & 91.99 & 88.44 & 90.10 & 81.60 \\\cline{2-2}\cline{4-10}
    & Transformer & & 72.66 & 79.71 & \underline{75.65} & 91.30 & 87.97 & 89.56 & \underline{82.61} \\\hline\hline
    
    \multirow{4}{*}{\bfseries Jointly trained} & GG-NN & \multirow{4}{*}{\shortstack[c]{Max / Mean /\\Self-attention}} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx  \\\cline{2-2}\cline{4-10}
    & RNN & & 94.75 & 94.78 & 94.76 & 89.17 & 89.07 & 89.11 & 91.94 \\\cline{2-2}\cline{4-10}
    & Bi-RNN & & 93.98 & 95.37 & 94.66 & 88.20 & 87.34 & 87.75 & 91.21 \\\cline{2-2}\cline{4-10}
    & Transformer & & 94.39 & 95.73 & \underline{95.04} & 90.35 & 88.48 & \underline{89.40} & \underline{\textbf{92.22}} \\\hline
  \end{tabular}
\end{table*}

\begin{table*}[!h]
  \centering
  \caption{Anomaly detection performance of proposed models}
  \label{tbl:detection_1}
  \begin{tabular}{|cc|ccc|ccc|ccc|}
    \hline
      \multicolumn{2}{|c|}{\bfseries Model} & \multicolumn{3}{|c|}{\bfseries WSD} & \multicolumn{3}{|c|}{\bfseries LAD1} & \multicolumn{3}{|c|}{\bfseries LAD2} \\
    \hline
    \bfseries Encoder & \bfseries Readout & \bfseries Precision & \bfseries Recall & \bfseries F1-measure & \bfseries Precision & \bfseries Recall & \bfseries F1-measure & \bfseries Precision & \bfseries Recall & \bfseries F1-measure \\
    \hline
    \multicolumn{11}{|c|}{Baseline models} \\\hline
    Raw features & Max & 0.9074 & 0.9103 & 0.9089 & 0.8804 & 0.8608 & 0.8702 & 0.8614 & 0.8218 & 0.8407  \\
    DNN & Max & 0.9565 & 0.9497 & 0.9531 & 0.9453 & 0.9288 & 0.9370 & 0.8986 & 0.9046 & 0.9012  \\
    \hline
    \multicolumn{11}{|c|}{Proposed models} \\\hline
    GG-NN & Max & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx & 0.xxxx  \\
    RNN & Max & 0.9581 & 0.9452 & 0.9516 & 0.9612 & 0.9135 & 0.9368 & 0.9001 & 0.8775 & 0.8878  \\
    Bi-RNN & Max & 0.9559 & 0.9489 & 0.9523 & 0.9456 & 0.9144 & 0.9296 & 0.9091 & 0.8939 & 0.9014  \\
    Transformer & Max & 0.9567 & 0.9510 & \textbf{0.9538} & 0.9682 & 0.9173 & \textbf{0.9421} & 0.9298 & 0.8780 & \textbf{0.9031}  \\\hline
  \end{tabular}
\end{table*}

% experiment result - table and graphics
\begin{table}[h!] \centering	
\caption{Scalability of proposed models on WSD dataset. All experiment results are in table \ref{tbl:scalability_2}}
    \label{tbl:scalability_1}
    \begin{tabular}{| l | r | r | r | r |}
    \hline
    \textbf{ Model } & \textbf{ default } & \textbf{ method 1 } & \textbf{ method 2 } \\\hline \hline
   Raw features & 93.96 & 64.37 & 90.52 \\
   DNN & \textbf{95.41} & 70.33 & 95.12 \\
   GG-NN & 94.06 & xx.xx & 94.25 \\ % result from [20.12.24.exp2, 21.02.11 exp7]
   RNN & 95.21 & 69.72 & 95.00 \\
   Bi-RNN & 95.23 & \textbf{73.28} & 94.83 \\
   Transformer & 95.38 & 72.83 & \textbf{95.20} \\
   \hline
   \end{tabular}
\end{table}


\begin{table*}[!h]
  \centering
    \caption{Scalability evaluation results for different models}
    \label{tbl:scalability_2}
  \begin{tabular}{|c|c|c|ccc|ccc|c|}
    \hline
      \multirow{3}{*}{\bfseries Training dataset} & \multirow{3}{*}{\bfseries Encoder} & \multirow{3}{*}{\bfseries Readout} & \multicolumn{6}{|c|}{\bfseries Test dataset} & \multirow{3}{*}{\shortstack[*]{\bfseries Average\\\bfseries F1-measure}} \\
      \cline{4-9}
      & & & \multicolumn{3}{|c|}{\bfseries WSD} & \multicolumn{3}{|c|}{\bfseries LAD2} & \\
    \cline{4-9}
    % \bfseries Testset  & \bfseries Encoder & \bfseries Readout 
    & & & \bfseries Precision & \bfseries Recall & \bfseries F1-measure & \bfseries Precision & \bfseries Recall & \bfseries F1-measure & \\
    \hline\hline
    
    \multirow{4}{*}{\bfseries WSD} & Raw features & \multirow{4}{*}{\shortstack[c]{Max / Mean /\\Self-attention }} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\\cline{2-2}\cline{4-10}
    & DNN & & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx\\\cline{2-2}\cline{4-10}
    & GG-NN & & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx\\\cline{2-2}\cline{4-10}
    & RNN & & 95.45 & 94.60 & 95.02 & 78.37 & 70.59 & 74.25 & 84.64\\\cline{2-2}\cline{4-10}
    & Bi-RNN & & 95.41 & 95.10 & 95.25 & 78.85 & 70.63 & \underline{74.50} & \underline{84.88} \\\cline{2-2}\cline{4-10}
    & Transformer & & 95.34 & 95.42 & \textbf{95.38} & 71.41 & 71.40 & 71.24 & 83.31  \\\hline\hline
    
    \multirow{4}{*}{\bfseries LAD2} & GG-NN & \multirow{4}{*}{\shortstack[c]{Max / Mean /\\Self-attention}} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\\cline{2-2}\cline{4-10}
    & RNN & & 68.33 & 80.23 & 73.79 & 93.36 & 87.94 & \underline{\textbf{90.55}} & 82.17  \\\cline{2-2}\cline{4-10}
    & Bi-RNN & & 65.79 & 82.27 & 73.09 & 91.99 & 88.44 & 90.10 & 81.60 \\\cline{2-2}\cline{4-10}
    & Transformer & & 72.66 & 79.71 & \underline{75.65} & 91.30 & 87.97 & 89.56 & \underline{82.61} \\\hline\hline
    
    \multirow{4}{*}{\bfseries Jointly trained} & GG-NN & \multirow{4}{*}{\shortstack[c]{Max / Mean /\\Self-attention}} & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx  \\\cline{2-2}\cline{4-10}
    & RNN & & 94.75 & 94.78 & 94.76 & 89.17 & 89.07 & 89.11 & 91.94 \\\cline{2-2}\cline{4-10}
    & Bi-RNN & & 93.98 & 95.37 & 94.66 & 88.20 & 87.34 & 87.75 & 91.21 \\\cline{2-2}\cline{4-10}
    & Transformer & & 94.39 & 95.73 & \underline{95.04} & 90.35 & 88.48 & \underline{89.40} & \underline{\textbf{92.22}} \\\hline
  \end{tabular}
\end{table*}

%Since there have been success in applying data-driven approach to building anomaly detection system using deep learning, it is natural to take a step toward developing more advanced deep learning models which have potential to provide stronger performance as well as desirable properties for ADS. Our approach adopts relatively recent advances in deep learning, and apply these model in order to increase the performance as well as providing extra ability to become more useful models in both supervised and unsupervised learning settings.

%There have been many previous works which employed data-driven approach. It is natural to take a step toward developing more advanced deep learning models which have potential to provide stronger performance as well as desirable properties for ADS. Our approach adopts relatively recent advances in deep learning, and apply these model in order to increase the performance as well as providing extra ability to become more useful models. We have applied various deep learning models for supervised anomaly detection task in virtual network function domain. Especially, we adopt bidirectional RNNs and Transformer network, which are widely used in natural language processing domain. Then we apply self-attention mechanism to provide scalability to our anomaly detection model. The proposed model provides strong performance compared to baselines as well as generalize to Service function chain (SFC) with varying number of nodes.
